The design of the n2EDM experiment

We present the design of a next-generation experiment, n2EDM, currently under construction at the ultracold neutron source at the Paul Scherrer Institute (PSI) with the aim of carrying out a high-precision search for an electric dipole moment of the neutron. The project builds on experience gained with the previous apparatus operated at PSI until 2017, and is expected to deliver an order of magnitude better sensitivity with provision for further substantial improvements. An overview is given of the experimental method and setup, the sensitivity requirements for the apparatus are derived, and its technical design is described.

==> packages.tex <==

\usepackage[T1]{fontenc}
%\usepackage{fourier}
\usepackage{lmodern}
%\usepackage[scaled=0.875]{helvet} % sansSerif
%\renewcommand{\ttdefault}{lmtt} %tt   font for typewriter
\usepackage[official,right]{eurosym}
\usepackage{textcomp}   % provides proper micro- and degree-symbol
\usepackage{gensymb}
%\usepackage[latin1]{inputenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[dvipsnames,pdftex]{xcolor}
\usepackage[pdftex]{graphicx,epsfig}
\usepackage{rotating}
\usepackage{wrapfig}
\usepackage{epsf}
\usepackage{fancybox}
%\usepackage{amsmath,amsthm,amssymb,amsfonts} %% too many math alphabets! DRi
\usepackage{amsmath,amsthm}
\usepackage{dsfont}\let\mathbb\mathds
\usepackage[hyphens]{url}
\usepackage[breaklinks=true,hidelinks]{hyperref}
%\usepackage[breaklinks=true]           {hyperref}   %better for final layouting: to find link to figures in text
\usepackage[section]{placeins} %allows to have unlimited floats
\usepackage{needspace}
\usepackage[suffix='']{epstopdf}
\usepackage{epigraph}
\usepackage[font=small,margin=1cm]{caption}
\usepackage{subfig}
\usepackage[percent]{overpic}
\usepackage{multicol}
\usepackage{multirow}
%%\usepackage{fixltx2e}
\usepackage{MnSymbol}
\usepackage[tight,nice]{units}
\usepackage{xspace}
\usepackage{pbox}
%\usepackage{isotope}
%\usepackage{tikz} %added for Victor
%\usepackage[markers,nolists]{endfloat} %zc, for editing 2013-12-23
%\usepackage{float}%added for Victor
\usepackage{siunitx}%added by Martin
\usepackage{enumitem}%added by jochen to get rid of space above itemize and enumerate environments

%\usepackage[mathletters]{ucs}  % Michal
%\usepackage[utf8]{inputenc}
%\usepackage{graphicx}


\usepackage{titlesec}
\usepackage{afterpage}

% from Romain Virot
%\usepackage{multirow}
%\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{upgreek}
%\usepackage{wasysym}
%\usepackage{siunitx}
%\usepackage{enumitem}
%\usepackage[super]{nth}
% end of Romain's packages

%
% from GUillaume
%\usepackage{amsmath,amsthm} %,amssymb}
%\usepackage{multirow}
%\usepackage{graphicx}
%\usepackage{upgreek}
% end GP


% we get error:  "PDF icnlusion  multiple pdfs with page group included in a single page"'
%usepackage{silence }  does not help for  this  (because it is pdflatex low level??) 
% maybe use  gs  on those files  (all pdf with transparency,  including those via gnuplot pdfcairo)
%http://tex.stackexchange.com/questions/76273/multiple-pdfs-with-page-group-included-in-a-single-page-warning
%or we can use LuaLaTex  (but then we should get rid of package epstopdf
%or is it my pdflatex?  MiKTeX-pdfTeX 2.9.4902 (1.40.14) (MiKTeX 2.9 64-bit)     22.06.2013  22:16

